ToolRL: Reward is All Tool Learning Needs

Current Large Language Models (LLMs) often undergo supervised fine-tuning (SFT) to acquire tool use capabilities. However, SFT struggles to generalize to unfamiliar or complex tool use scenarios. Recent advancements in reinforcement learning (RL), particularly with R1-like models, have demonstrated promising reasoning and generalization abilities. Yet, reward design for tool use presents unique challenges: multiple tools may be invoked with diverse parameters, and coarse-grained reward signals, such as answer matching, fail to offer the finegrained feedback required for effective learning. In this work, we present the first comprehensive study on reward design for tool selection and application tasks within the RL paradigm. We systematically explore a wide range of reward strategies, analyzing their types, scales, granularity, and temporal dynamics. Building on these insights, we propose a principled reward design tailored for tool use tasks and apply it to train LLMs using Group Relative Policy Optimization (GRPO). Empirical evaluations across diverse benchmarks demonstrate that our approach yields robust, scalable, and stable training, achieving a 17% improvement over base models and a 15% gain over SFT models. These results highlight the critical role of thoughtful reward design in enhancing the tool use capabilities and generalization performance of LLMs. All the codes are released to facilitate future research.

==> tables/data_overall.tex <==
% rlla-grpo-qwen2.5-3b-ins4knolength-withkl-coarsereward & 53.93\% & 82.79\% & 80.55\% & 72.37\% & 7.25\% & 88.89\% & 81.67\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-schedulereward & 53.81\% & 81.44\% & 80.75\% & 75.43\% & 3.62\% & 77.78\% & 88.82\% \\
% rlla-grpo-qwen2.5-3b-ins4k-withkl & 53.22\% & 82.98\% & 80.50\% & 70.15\% & 7.38\% & 88.89\% & 77.57\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-withkl-correctmax1 & 52.99\% & 82.54\% & 75.52\% & 72.28\% & 6.62\% & 83.33\% & 81.35\% \\
% rlla-grpo-qwen2.5-3b-ins4k-nolength & 52.98\% & 81.58\% & 79.43\% & 73.78\% & 3.75\% & 88.24\% & 84.85\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-withkl-strictmatch & 52.81\% & 81.00\% & 80.80\% & 71.75\% & 5.00\% & 83.33\% & 82.45\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-withkl-schedulereward & 52.51\% & 82.29\% & 78.80\% & 71.26\% & 5.12\% & 83.33\% & 79.99\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-withkl-max1step30max3 & 52.12\% & 82.46\% & 74.59\% & 71.66\% & 5.38\% & 94.44\% & 80.45\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-strictmatch & 52.06\% & 81.65\% & 79.64\% & 69.21\% & 5.50\% & 83.33\% & 78.14\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-correctmax1 & 51.76\% & 81.50\% & 79.50\% & 69.79\% & 4.25\% & 88.89\% & 78.07\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-coarsereward & 51.40\% & 79.48\% & 78.54\% & 68.73\% & 5.62\% & 88.89\% & 77.80\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-refinedreward & 51.36\% & 81.15\% & 80.07\% & 68.64\% & 4.25\% & 88.89\% & 75.74\% \\
% rlla-grpo-qwen2.5-3b-ins-nolength & 51.36\% & 81.56\% & 79.18\% & 65.33\% & 8.50\% & 94.12\% & 67.81\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-max1step30max3 & 50.66\% & 80.62\% & 78.82\% & 67.93\% & 3.50\% & 88.89\% & 76.42\% \\
% rlla-grpo-llama3.2-3b-ins4k-nolength & 50.50\% & 74.38\% & 75.18\% & 72.59\% & 1.37\% & 94.44\% & 97.92\% \\
% rlla-grpo-qwen2.5-3b-ins-schedulereward & 50.30\% & 81.71\% & 78.59\% & 63.47\% & 7.13\% & 88.24\% & 68.78\% \\
% rlla-grpo-qwen2.5-3b-ins4k-max1step30max3 & 49.69\% & 80.33\% & 79.57\% & 65.39\% & 3.25\% & 83.33\% & 75.08\% \\
% rlla-grpo-qwen2.5-3b-ins4k-strictmatch & 49.53\% & 78.98\% & 80.64\% & 64.59\% & 3.75\% & 83.33\% & 73.34\% \\
% rlla-grpo-qwen2.5-3b-ins4k-correctmax1 & 49.37\% & 80.73\% & 76.41\% & 64.59\% & 4.50\% & 83.33\% & 72.71\% \\
% rlla-grpo-qwen2.5-3b-ins4k-refinedreward & 49.17\% & 77.42\% & 80.04\% & 63.93\% & 4.62\% & 88.89\% & 69.50\% \\
% rlla-grpo-qwen2.5-3b-ins-new & 49.12\% & 77.67\% & 79.64\% & 61.56\% & 7.50\% & 100.00\% & 63.11\% \\
% rlla-grpo-qwen2.5-3b-ins4k-new & 48.89\% & 77.83\% & 78.61\% & 63.56\% & 4.50\% & 88.24\% & 71.22\% \\
% rlla-grpo-qwen2.5-3b-ins-max1step30max3 & 48.52\% & 79.25\% & 80.14\% & 58.84\% & 8.75\% & 100.00\% & 53.40\% \\
% rlla-grpo-qwen2.5-3b-ins-strictmatch & 48.39\% & 79.19\% & 77.46\% & 60.80\% & 6.50\% & 88.24\% & 62.31\% \\
% rlla-grpo-qwen2.5-3b-ins4k-schedulelength & 48.24\% & 77.60\% & 79.11\% & 63.22\% & 3.00\% & 88.89\% & 68.53\% \\
% rlla-grpo-qwen2.5-3b-ins-new & 48.18\% & 80.02\% & 78.39\% & 58.76\% & 7.75\% & 100.00\% & 55.58\% \\
% rlla-grpo-llama3.2-3b-ins4knolength-withkl-refinedreward & 47.84\% & 75.12\% & 76.30\% & 65.39\% & 2.88\% & 72.22\% & 75.06\% \\
% rlla-grpo-sft4k-qwen2.5-3b-ins4k-nolength & 47.82\% & 75.12\% & 69.52\% & 68.19\% & 2.38\% & 77.78\% & 76.16\% \\
% rlla-grpo-qwen2.5-3b-ins4k-schedulereward & 47.81\% & 79.83\% & 80.34\% & 60.51\% & 3.50\% & 94.44\% & 62.14\% \\
% rlla-grpo-qwen2.5-3b-ins-correctmax1 & 47.72\% & 77.94\% & 77.04\% & 58.18\% & 9.12\% & 94.12\% & 52.32\% \\
% rlla-grpo-qwen2.5-3b-ins4k-coarsereward & 47.58\% & 77.00\% & 75.04\% & 62.02\% & 4.13\% & 88.89\% & 69.99\% \\
% rlla-grpo-qwen2.5-3b-ins-coarsereward & 46.99\% & 77.21\% & 77.93\% & 57.29\% & 7.00\% & 88.24\% & 57.64\% \\
% rlla-grpo-llama3.2-3b-ins4knolength-withkl-schedulereward & 46.85\% & 83.00\% & 72.77\% & 61.00\% & 3.38\% & 88.89\% & 59.37\% \\
% rlla-grpo-sft400-qwen2.5-3b-ins4k-nolength & 46.42\% & 76.21\% & 68.93\% & 64.15\% & 1.75\% & 88.89\% & 71.76\% \\
% rlla-grpo-qwen2.5-1.5b-ins4knolength-withkl-strictmatch & 46.20\% & 78.92\% & 76.21\% & 61.08\% & 1.62\% & 100.00\% & 57.33\% \\
% rlla-grpo-qwen2.5-1.5b-ins4k-nolength & 46.20\% & 77.96\% & 76.98\% & 60.73\% & 2.25\% & 100.00\% & 56.44\% \\
% rlla-grpo-qwen2.5-3b-ins-refinedreward & 46.17\% & 78.75\% & 78.04\% & 55.51\% & 6.50\% & 100.00\% & 48.31\% \\
% rlla-grpo-qwen2.5-1.5b-ins4knolength-schedulereward & 45.71\% & 78.31\% & 75.73\% & 58.91\% & 2.50\% & 100.00\% & 57.20\% \\
% qwen2.5-3b-full-sft4k-checkpoint-711 & 45.61\% & 67.00\% & 66.71\% & 67.17\% & 1.62\% & 72.22\% & 76.90\% \\
% rlla-grpo-sft4k-llama3.2-3b-ins4k-nolength & 45.50\% & 70.69\% & 67.70\% & 64.73\% & 1.00\% & 77.78\% & 78.85\% \\
% rlla-grpo-llama3.2-3b-ins4knolength-withkl & 45.44\% & 74.52\% & 72.79\% & 61.08\% & 1.62\% & 88.89\% & 66.94\% \\
% qwen2.5-7b-full-rlla600-0309-checkpoint-201 & 45.32\% & 66.31\% & 62.38\% & 65.82\% & 4.87\% & 64.71\% & 69.70\% \\
% rlla-grpo-llama3.2-3b-ins4k-new & 44.98\% & 78.02\% & 77.54\% & 56.55\% & 1.25\% & 100.00\% & 63.76\% \\
% rlla-grpo-qwen2.5-1.5b-ins4knolength-withkl-schedulereward & 44.96\% & 79.00\% & 75.84\% & 57.09\% & 2.12\% & 100.00\% & 52.77\% \\
% qwen2.5-3b-full-sft400 & 44.63\% & 69.27\% & 66.32\% & 64.10\% & 1.00\% & 83.33\% & 71.78\% \\
% rlla-grpo-llama3.2-3b-ins4knolength-withkl-coarsereward & 44.41\% & 81.90\% & 70.52\% & 57.13\% & 2.75\% & 100.00\% & 47.26\% \\
% llama3.2-3b-full-sft4k-checkpoint-711 & 44.16\% & 65.42\% & 67.02\% & 63.04\% & 1.38\% & 77.78\% & 78.25\% \\
% rlla-grpo-llama3.2-3b-ins4k-correctmax1 & 44.12\% & 76.62\% & 76.00\% & 56.42\% & 0.38\% & 88.89\% & 63.53\% \\
% rlla-grpo-llama3.2-3b-ins4k-strictmatch & 43.84\% & 75.75\% & 76.34\% & 55.09\% & 1.25\% & 94.44\% & 60.58\% \\
% rlla-grpo-llama3.2-3b-ins4k-max1step30max3 & 43.20\% & 75.60\% & 71.34\% & 56.11\% & 1.75\% & 94.44\% & 56.00\% \\
% rlla-grpo-llama3.2-3b-ins4k-schedulelength & 43.15\% & 75.50\% & 71.64\% & 56.06\% & 1.00\% & 100.00\% & 57.82\% \\
% rlla-grpo-llama3.2-3b-ins4knolength-schedulereward & 42.84\% & 75.46\% & 76.11\% & 52.87\% & 2.00\% & 94.44\% & 51.07\% \\
% rlla-grpo-sft4k-qwen2.5-1.5b-ins4k-nolength & 42.63\% & 66.60\% & 64.77\% & 60.15\% & 1.38\% & 88.89\% & 67.98\% \\
% rlla-grpo-sft400-llama3.2-3b-ins4k-nolength & 42.54\% & 65.15\% & 68.98\% & 59.40\% & 0.88\% & 72.22\% & 65.80\% \\
% rlla-grpo-llama3.2-3b-ins4knolength-correctmax1 & 42.47\% & 67.77\% & 75.05\% & 55.75\% & 1.00\% & 88.89\% & 59.56\% \\
% Qwen2.5-7B-Instruct & 41.97\% & 66.02\% & 70.11\% & 53.51\% & 4.25\% & 76.47\% & 62.66\% \\
% rlla-grpo-llama3.2-3b-ins4knolength-max1step30max3 & 41.33\% & 65.54\% & 72.70\% & 55.22\% & 0.75\% & 88.89\% & 57.59\% \\
% llama3.2-3b-full-sft400 & 41.22\% & 64.27\% & 62.18\% & 58.37\% & 0.75\% & 66.67\% & 71.12\% \\
% rlla-grpo-qwen2.5-1.5b-ins4knolength-withkl & 41.13\% & 78.62\% & 74.75\% & 50.64\% & 1.00\% & 100.00\% & 28.34\% \\
% qwen2.5-3b-full-rlla600-0309-checkpoint-201 & 41.10\% & 63.00\% & 63.86\% & 58.80\% & 1.12\% & 76.47\% & 60.26\% \\
% rlla-grpo-sft400-qwen2.5-1.5b-ins4k-nolength & 40.93\% & 70.54\% & 60.79\% & 56.33\% & 1.00\% & 94.44\% & 58.63\% \\
% rlla-grpo-qwen2.5-1.5b-ins4knolength-strictmatch & 40.71\% & 78.00\% & 75.55\% & 48.91\% & 2.00\% & 100.00\% & 24.84\% \\
% qwen2.5-1.5b-full-sft4k-checkpoint-711 & 40.67\% & 59.94\% & 59.84\% & 59.31\% & 1.00\% & 88.89\% & 71.34\% \\
% qwen2.5-1.5b-full-sft400 & 40.21\% & 65.12\% & 61.11\% & 56.69\% & 1.00\% & 94.44\% & 60.14\% \\
% rlla-grpo-llama3.2-3b-ins4knolength-strictmatch & 39.82\% & 64.71\% & 70.68\% & 52.20\% & 0.25\% & 100.00\% & 56.68\% \\
% rlla-grpo-qwen2.5-1.5b-ins4knolength-correctmax1 & 39.47\% & 78.56\% & 75.50\% & 45.45\% & 2.50\% & 100.00\% & 16.44\% \\
% llama3.2-3b-full-rlla600-0309-checkpoint-201 & 39.03\% & 58.77\% & 58.54\% & 55.89\% & 1.00\% & 83.33\% & 68.62\% \\
% rlla-grpo-llama3.2-3b-ins4k-coarsereward & 38.98\% & 61.15\% & 65.54\% & 51.98\% & 1.12\% & 77.78\% & 61.68\% \\
% rlla-grpo-qwen2.5-1.5b-ins4knolength-max1step30max3 & 38.85\% & 77.96\% & 76.23\% & 44.51\% & 2.25\% & 100.00\% & 10.61\% \\
% rlla-grpo-llama3.2-3b-ins4knolength-refinedreward & 38.62\% & 59.83\% & 71.86\% & 50.56\% & 0.25\% & 94.44\% & 55.68\% \\
% rlla-grpo-qwen2.5-1.5b-ins4knolength-refinedreward & 37.65\% & 77.94\% & 72.46\% & 43.00\% & 1.62\% & 100.00\% & 12.45\% \\
% rlla-grpo-qwen2.5-1.5b-ins4knolength-coarsereward & 36.72\% & 76.44\% & 70.86\% & 41.27\% & 2.12\% & 100.00\% & 12.24\% \\
% rlla-grpo-llama3.2-3b-ins4knolength-coarsereward & 35.95\% & 52.00\% & 61.43\% & 48.96\% & 1.12\% & 83.33\% & 61.92\% \\
% rlla-grpo-qwen2.5-1.5b-ins4k-new & 33.23\% & 70.58\% & 71.36\% & 35.63\% & 0.50\% & 94.44\% & 4.52\% \\
% Qwen2.5-3B-Instruct & 33.04\% & 42.52\% & 40.80\% & 53.96\% & 1.00\% & 64.71\% & 56.01\% \\
% Llama-3.1-8B-Instruct & 30.71\% & 39.40\% & 36.41\% & 52.29\% & 0.38\% & 94.44\% & 46.62\% \\
% rlla-grpo-qwen2.5-1.5b-ins4k-schedulelength & 28.51\% & 53.23\% & 48.23\% & 38.07\% & 0.00\% & 55.56\% & 25.08\% \\
% Llama-3.2-3B-Instruct & 22.09\% & 17.44\% & 14.57\% & 43.85\% & 0.00\% & 77.78\% & 66.07\% \\
% Qwen2.5-1.5B-Instruct & 19.41\% & 16.00\% & 13.18\% & 35.58\% & 0.00\% & 44.44\% & 82.49\% \\
% rlla-grpo-qwen2.5-1.5b-ins4knolength-withkl-refinedreward & 16.76\% & 0.00\% & 0.00\% & 39.18\% & 0.00\% & 0.00\% & 100.00\% \\
% rlla-grpo-qwen2.5-3b-ins4knolength-withkl & 16.76\% & 0.00\% & 0.00\% & 39.18\% & 0.00\% & 0.00\% & 100.00\% \\
